From Handcrafted Features to LLMs: A Brief Survey for Machine Translation Quality Estimation

Machine Translation Quality Estimation (MTQE) is the task of estimating the quality of machine-translated text in real time without the need for reference translations, which is of great importance for the development of MT. After two decades of evolution, QE has yielded a wealth of results. This article provides a comprehensive overview of QE datasets, annotation methods, shared tasks, methodologies, challenges, and future research directions. It begins with an introduction to the background and significance of QE, followed by an explanation of the concepts and evaluation metrics for word-level QE, sentence-level QE, document-level QE, and explainable QE. The paper categorizes the methods developed throughout the history of QE into those based on handcrafted features, deep learning, and Large Language Models (LLMs), with a further division of deep learning-based methods into classic deep learning and those incorporating pre-trained language models (LMs). Additionally, the article details the advantages and limitations of each method and offers a straightforward comparison of different approaches. Finally, the paper discusses the current challenges in QE research and provides an outlook on future research directions.

==> IJCNN____________.tex <==
为了使你的方程更紧凑，你可以使用斜杠（~/~）、exp函数或适当的指数。将表示数量和变量的罗马符号斜体化，但希腊符号除外。
使用长破折号而不是连字符来表示负号。当方程是句子的一部分时，用逗号或句号进行标点，如下所示： \begin{equation} a+b=\gamma\label{eq} \end{equation}
 
确保你的方程中的符号在方程之前或紧接方程后已被定义。
使用{eq}''，而不是Eq.~\eqref{eq}''或equation \eqref{eq}''，除非在句子开头：Equation \eqref{eq} 是 . . .''
           


请使用软引用（例如，\verb|\eqref{Eq}|）交叉引用而不是硬''引用（例如，\verb|(1)|）。这将使得合并章节、添加方程或更改图表或引文的顺序成为可能，而不需要逐行检查文件。
 
请不要使用\verb|{eqnarray}|方程环境。请使用\verb|{align}|或\verb|{IEEEeqnarray}|代替。因为\verb|{eqnarray}|环境会在关系符号周围留下不雅观的空间。
请注意，{\LaTeX}中的\verb|{subequations}|环境即使在没有显示方程编号的情况下也会增加主方程计数器。如果你忘记了这一点，你可能会写出一个方程编号从（17）跳到（20）的文章，使得校对编辑想知道你是否发现了一种新的计数方法。
{\BibTeX}并非魔法般工作。它不是从空气中获取参考文献数据，而是从.bib文件中获取。如果您使用{\BibTeX}生成参考文献列表，您必须发送.bib文件。
{\LaTeX}无法读懂你的心思。如果你给一个小节和一个表格分配相同的标签，你可能会发现表格I被交叉引用为表格IV-B3。
{\LaTeX}没有先知能力。如果你在更新计数器的命令之前放置了一个\verb|\label|命令，标签将捕获最后一个被交叉引用的计数器。特别是，\verb|\label|命令不应该放在图形或表格的标题之前。
不要在\verb|{array}|环境内使用\verb|\nonumber|。它不会阻止\verb|{array}|内的方程编号（反正不会有任何编号），并且它可能会阻止周围方程中所需的方程编号。


一些命令错误
	data是复数，而不是单数
	下标，应该是数字零的下标格式，而不是小写字母“o”
	在美式英语中，逗号、分号、句号、问号和感叹号只有在引用完整的，如标题或完整引文时，才位于引号内。当引号被用来强调单词或短语而不是用粗体或斜体时，标点符号应该出现在引号外面。句子末尾的括号内的附加短语或声明的标点符号应该位于闭括号的外面（像这样）。(括号内的完整句子在括号内标点。)  
	图中的小图被称为“嵌图”，而不是“插图”。词汇“alternatively”(另外)优于“alternately”（除非你真的指交替）
	不要使用单词essentially''来表示大约''或实际上 
	在您的论文标题中，如果短语“that uses”可以准确地替换单词“using”，则将“u”字母大写；如果不行，则继续使用小写字母。
	注意同音异义词“affect”和“effect”、“complement”和“compliment”、“discreet”和“discrete”、“principal”和“principle”的不同含义
	不要混淆“imply”和“infer”。
	前缀“non”不是一个单词；它应该与它所修饰的词连用，通常不需要连字符。
	拉丁文缩写“et al.”中的“et”后面没有句点
	缩写“i.e.”的意思是“即”，缩写“e.g.”的意思是“例如”


该类文件的设计是为了六位作者使用，但不仅限于此。所有会议文章至少需要一位作者。作者姓名应从左到右列出，然后移到下一行继续。这将是将来引用和索引服务中使用的作者顺序。姓名不应按列排列，也不应按隶属关系分组。请尽量保持您的隶属关系简洁（例如，不要在同一组织的不同部门之间做区分）。


标题或称为头部，是组织性的工具，指导读者阅读您的论文。有两种类型：组件头和文本头。
组件头用于识别论文的不同组成部分，并且彼此之间在主题上不是从属关系。示例包括“致谢”和“参考文献”，对于这些，正确的样式是使用“Heading 5”。对于图表的标题说明，请使用“figure caption”，对于表格的标题，请使用“table head”。像“摘要”这样的内文标题，需要你额外应用一种样式（在这个例子中，是斜体），以便通过下拉菜单提供的样式将标题与文本区分开来。
文本头按照关系性、层次性的基础来组织主题。例如，论文标题是主要的文本头，因为所有后续材料都与这个主题相关并进行阐述。如果有两个或多个子主题，应使用下一级标题（大写罗马数字）。相反，如果没有至少两个子主题，那么就不应该引入子标题。


图表和表格的摆放位置：将图形和表格置于栏目的顶部和底部。避免将它们放置在栏目的中间。大型图形和表格可能跨越两个栏目。图形说明应该放在图形下方；表头应该出现在表格上方。在文中引用图形和表格之后再插入它们。即使在句子的开头，也使用缩写“图 1”。 Fig.~\ref{fig}    
.
.


图形标签：使用8号Times New Roman字体作为图形标签。在编写图形轴标签时，使用文字而非符号或缩写，以避免让读者感到困惑。例如，写出“磁化强度”或“磁化强度, M”，而不是仅仅写“M”。如果标签中包含单位，应将单位放在括号内。不要仅用单位来标记轴。在该例中，写“磁化强度 (A/m)”或“磁化强度 {A[m(1)]}”，而不是仅写“A/m”。不要用数量与单位的比率来标记轴。例如，写“温度 (K)”，而不是“温度/K”。
 


在美国，“致谢”这个词的首选拼写是在“g”之后没有额外的“e”。避免使用生硬的表达方式“我们中的一个人（R. B. G.）感谢……”。相反，尝试使用“R. B. G. 感谢……”。将赞助者的致谢放在第一页的无编号脚注中。

  




请在括号内连续对引用进行编号[1]。句子的标点符号应该放在括号[2]之后。简单地指代参考文献号码，如[3]——不要使用“参考文献[3]”或“文献[3]”，除非是句子的开头：“文献[3]是第一个……”
脚注在上标中分别编号。将实际的脚注放在引用它的那一栏的底部。不要在摘要或参考文献列表中放置脚注。表格脚注请使用字母。
除非有六位或更多作者，否则请给出所有作者的姓名；不要使用“等”。即使已经提交发表的论文，如果尚未发表，应该被引用为“未发表”[4]。已被接受发表的论文应该被引用为“在审”[5]。在论文标题中，仅将首个单词大写，专有名词和元素符号除外。
对于在翻译期刊上发表的论文，请首先给出英文引用，然后是原始的外语引用[6]。



